Modeling Thousands of Human Annotators for Generalizable Text-to-Image Person Re-identification

Text-to-image person re-identification (ReID) aims to retrieve the images of an interested person based on textual descriptions. One main challenge for this task is the high cost in manually annotating large-scale databases, which affects the generalization ability of ReID models. Recent works handle this problem by leveraging Multi-modal Large Language Models (MLLMs) to describe pedestrian images automatically. However, the captions produced by MLLMs lack diversity in description styles. To address this issue, we propose a Human Annotator Modeling (HAM) approach to enable MLLMs to mimic the description styles of thousands of human annotators. Specifically, we first extract style features from human textual descriptions and perform clustering on them. This allows us to group textual descriptions with similar styles into the same cluster. Then, we employ a prompt to represent each of these clusters and apply prompt learning to mimic the description styles of different human annotators. Furthermore, we define a style feature space and perform uniform sampling in this space to obtain more diverse clustering prototypes, which further enriches the diversity of the MLLM-generated captions. Finally, we adopt HAM to automatically annotate a massive-scale database for text-to-image ReID. Extensive experiments on this database demonstrate that it significantly improves the generalization ability of ReID models.

==> rebuttal.tex <==
% \documentclass[10pt,twocolumn,letterpaper]{article}
% \usepackage[rebuttal]{cvpr}

% % Include other packages here, before hyperref.
% \usepackage{graphicx}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{booktabs}

% Import additional packages in the preamble file, before hyperref
\input{preamble}

\clearpage
\setcounter{page}{1}

% If you comment hyperref and then uncomment it, you should delete
% egpaper.aux before re-running latex.  (Or just hit 'q' on the first latex
% run, let it finish, and you should be clear).
\definecolor{cvprblue}{rgb}{0.21,0.49,0.74}
% \usepackage[pagebackref,breaklinks,colorlinks,citecolor=cvprblue]{hyperref}

% Support for easy cross-referencing
% \usepackage[capitalize]{cleveref}
\crefname{section}{Sec.}{Secs.}
\Crefname{section}{Section}{Sections}
\Crefname{table}{Table}{Tables}
\crefname{table}{Tab.}{Tabs.}

% If you wish to avoid re-using figure, table, and equation numbers from
% the main paper, please uncomment the following and change the numbers
% appropriately.
%\setcounter{figure}{2}
%\setcounter{table}{1}
%\setcounter{equation}{2}

% If you wish to avoid re-using reference numbers from the main paper,
% please uncomment the following and change the counter for `enumiv' to
% the number of references you have in the main paper (here, 6).
%\let\oldthebibliography=\thebibliography
%\let\oldendthebibliography=\endthebibliography
%\renewenvironment{thebibliography}[1]{%
%     \oldthebibliography{#1}%
%     \setcounter{enumiv}{6}%
%}{\oldendthebibliography}


%%%%%%%%% PAPER ID  - PLEASE UPDATE
\def\paperID{6365} % *** Enter the Paper ID here
\def\confName{CVPR}
\def\confYear{2024}

% \begin{document}

%%%%%%%%% TITLE - PLEASE UPDATE

% \maketitle
% \thispagestyle{empty}
\appendix

%%%%%%%%% BODY TEXT - ENTER YOUR RESPONSE BELOW
\noindent{\textbf{\color{blue} Response To All Reviewers:}}
% Thanks to all the reviewers and AC for your constructive comments. 
We thank {\textbf{\color{cyan}{R1}}} ({\textbf{\color{cyan}{z1sG}}}), {\textbf{\color{green}{R2}}} ({\textbf{\color{green}{PDvd}}}), {\textbf{\color{orange}{R3}}} ({\textbf{\color{orange}{68W7}}}) and AC for your valuable comments. 
The reviewers regard our method as \textbf{novel}~[{\textbf{\color{green}{R2}}}, {\textbf{\color{orange}{R3}}}], \textbf{clearly motivated}~[{\textbf{\color{green}{R2}}}], \textbf{efficient}~[{\textbf{\color{green}{R2}}}, {\textbf{\color{orange}{R3}}}], the idea \textbf{makes sense}~[{\textbf{\color{orange}{R3}}}]; 
experimental results are \textbf{extensive}~[{\textbf{{\color{orange}{R3}}}] and \textbf{promising}~[{\textbf{\color{green}{R2}}}], the improvement is \textbf{substantial}~[{\textbf{\color{orange}{R3}}}]; 
the paper is \textbf{well-organized}~[{\textbf{\color{green}{R2}}}], \textbf{well-written}~[{\textbf{{\color{green}{R2}}}, {\textbf{\color{orange}{R3}}}}], and \textbf{easy to follow}~[{\textbf{\color{green}{R2}}}, {\textbf{\color{orange}{R3}}}}], the illustrations are \textbf{clearly depicted}~[{\textbf{\color{green}{R2}}}] and \textbf{nice}~[{\textbf{\color{orange}{R3}}}].
% is \textbf{effective}~{\color{cyan}{[Dq8H]}}, \textbf{easily adapted}~{\color{cyan}{[Dq8H,MvjH,SaQA]}} and \textbf{rational}~{\color{cyan}{[SaQA]}};the performance increase is \textbf{impressive} {\color{cyan}{[Dq8H,MvjH,SaQA]}}; the paper is \textbf{extremely well-written}~{\color{cyan}{[MvjH]}} and \textbf{easily comprehensible}~{\color{cyan}{[MvjH,SaQA]}}.

% Reviewer 1
\noindent{\textbf{\color{cyan} Response To R1:}}
\noindent{\underline{\textbf{\color{cyan} Q1:}}}
%Comparison with different preference prompts given to LLM 
The necessity of HAM.
\noindent{\underline{\textbf{\color{cyan} A1:}}}
Table 1 (1)-(3) show that increasing the number of templates (from 46K to 68K) leads to a performance bottleneck, indicating even with different prompts, the diversity of LLM outputs is quite limited. One reason is template use losing stylistic information (e.g., granularity and word preferences) as we explain in L. 52-54. Another reason is the lack of human-annotated prior knowledge; the LLM's outputs tend to rely on the long-tail data distribution from its training, leading to biased sentence structures and word styles [DOI:10.48550/arXiv.2409.03025, DOI:10.48550/arXiv.1710.02534], and fails to align with human descriptive styles. Therefore, it is essential to use our HAM to exploit MLLM diversity in pedestrian descriptions. Comparing unique word counts, CUHK-PEDES has 9,409 words, while LLaVA1.6 (untrained and trained with HAM) generates 5,332 and 7,402 words, respectively, highlighting an increase in diversity. However, we acknowledge that unique word count alone doesn't fully measure diversity. As for the count of sentence patterns, it remains challenging but we believe this does not diminish the evidence from experiments (1) and (11) in Table 1, which clearly show the improved caption diversity using our method.
%Though LLM can yield diverse descriptions based on the different prompt, the experiment result in Table1 46Td compared with 68k Td shows that the improvement(多样性提升) of diverse prompts quickly reach a limit（很快达到瓶颈）。原因一个是用template会丢失很多风格信息比如被去掉的属性描述的描述粒度和word偏好，能代表的风格内容很有限，正如我们在文中第x行所说；另一个原因是在缺乏人类先验知识，llm的输出会依赖于训练时的长尾数据分布导致输出有偏向的句式和word style[引用]，缺乏与人类描述风格的对齐。 所以it is necessary to use our HAM to 挖掘llm对行人描述的多样性。We also count the number of unique words in existing dataset且结果如下：CUHK has 1000 unique而ICFG有200个，rstp有200个。而相同数量文本下（1M）未经训练的llava和使用我们方法HAM微调之后的caption分别有100和200个unique words，which shows 我们方法对自动标注数据多样性的提升，尽管我们指出单独看unique word并不能全方面地衡量多样性。且the number of sentence pattern in现有数据集是不重要的，因为从表1的实验x（）中我们使用数据集中所有的template来让mllm产生caption也只得到了有限的提升，对比我们的方法而言（）

\noindent{\underline{\textbf{\color{cyan} Q2:}}}
Consideration on the diversity constraints of existing datasets.
\noindent{\underline{\textbf{\color{cyan} A2:}}}
In Table 1, we use the MLLM to learn descriptive styles only from the CUHK-PEDES dataset, while also demonstrating significant performance improvements on the ICFG-PEDES and RSTP-ReID. This indicates that learning human stylistic diversity from one existing dataset can generalize to other unseen datasets, offering a solution to the limitation of a small number of templates.
%In our experiment in Tabel 1, we only employ the MLLM to learn and mimic the descriptive styles in CUHK-PEDES dataset and also show the significant improvement in ICFG as well as RSTP datasets. 这表明即使从单独一个现有数据集中学习人类风格多样性也能泛化到其他未见数据集的风格，而不是只限于训练数据集所拥有的风格多样性。So 这也是我们提出用来solve the problem of limited number of templates的方法。
\noindent{\underline{\textbf{\color{cyan} Q3:}}}
The definition of the text description style.
\noindent{\underline{\textbf{\color{cyan} A3:}}}
Our definition of descriptive style includes sentence pattern, wording style, granularity and order of descriptions and so on. We replace only pedestrian-specific words in the descriptions, preserving stylistic information. After text encoding, we extract stylistic features, allowing us to cluster sentences with similar styles. The reliability of this approach is demonstrated by the visualization(Figure E), where captions for different pedestrian images, given the same style prompt, consistently exhibit similar sentence patterns, granularity, and wording style.
%相比起之前工作{}只关注句式多样性，我们所定义的描述风格还包含了wording style and 描述粒度（such as xxx or xxx）等方面。我们只将描述中有辨别性的word替换，得到尽可能保留风格信息的风格句子，经过文本编码之后得到了我们要提取的风格特征。依靠这些特征我们可以将风格相似的句子聚类在一起。The reliability 证明可以从我们附录中展示的可视化结果中看出，基于相同的prompt给不同行人图像打的cap在描述句式、描述粒度和word style上高度一致。

\noindent{\underline{\textbf{\color{cyan} Q4:}}}
More ablation study results.
\noindent{\underline{\textbf{\color{cyan} A4:}}}
The results are shown in the table below, which also demonstrates the effectiveness of our method and the reasonableness of the hyper-parameters.

\begin{table}[h]
\vspace{-1em}
\resizebox{0.475\textwidth}{!}{%
\begin{tabular}{c|c|c|c}
\hline
Method & CUHK-PEDES & ICFG-PEDES & RSTPReid \\ \hline
HAM+DBSCAN+UPS & 57.71/51.64  &34.97/18.38  &48.10/35.61  \\
% IRRA+4cap & 73.97  &66.76  &  &  &  &  \\
HAM+KMeans+UPS($K_1=2000,K_2=2000$) &59.92/53.62  & 36.09/18.86  &50.75/36.89  \\ \hline
\end{tabular}}
\vspace{-1.5em}
\end{table}

\noindent{\underline{\textbf{\color{cyan} Q5:}}}
The measurement of the style diversity in obtained descriptions.
\noindent{\underline{\textbf{\color{cyan} A5:}}}
In response to R1Q1, we count the unique words in descriptions with and without our method. However, this only captures a limited aspect of style diversity. While fully quantifying style diversity is challenging, we believe it is not critical because the overall quality of the captions including the diversity can be reflected in the ReID model performance trained with these descriptions.
%正如我们在R1Q1中回答的，我们计算了通过我们的方法得到的descriptions和不使用我们方法的description的unique word数量，但这只能代表风格多样性的其中一方面。对风格多样性的整体量化是抽象的但我们认为这并不重要，因为我们最终可以从使用了这些描述来训练的reid模型性能中反映出其总体多样性质量。

\noindent{\underline{\textbf{\color{cyan} Q6:}}}
More implementation details.
\noindent{\underline{\textbf{\color{cyan} A6:}}}
As explained in the Method section, integrating our approach with different MLLMs only requires adding the learnable prompt module and fine-tune the vision-language adaptor simultaneously. This enables the implementation of our method across various MLLMs. Table 1 shows the HAM's performance on LLaVA-1.6 and Qwen-VL, and, as mentioned in our reply to R3Q3, we also provide results for MiniCPM-V 2.5.
%正如我们在Method章节中展示的一样，To be integrated with 不同的MLLMs, 我们只需要添加learnable prompt module to different MLLMs and 同时微调 vision-language adaptor即可在不同的MLLM中实现我们的方法。我们的实验中亦给出了HAM在Llava1.6和QwenVL这两种模型上的性能如表1所示。

% Reviewer 2
\noindent{\textbf{\color{green} Response To R2:}}
\noindent{\underline{\textbf{\color{green} Q1:}}}
The number of clusters. 
\noindent{\underline{\textbf{\color{green} A1:}}}
We have provided the hyper-parameter experiments and related explanations in Figure B and Table A of the supplement, which validate the choice of hyper-parameters used. Hope this clear your concerns.
%We have included the hyper-parameter experiments and explanation related to the clustering method in the Figure B and Table A in the supplement. These results validate the reasonableness of the hyper-parameters we used.
%感谢您的宝贵意见。由于正文篇幅限制的原因我们将关于聚类方法的超参实验，包括number of cluster used in KMeans and UPS, as well as the number of samples in each UPS cluster都放在附录中，如附录的Figure B 和 Table A所示并证实了我们选用的超参的合理性。
\noindent{\underline{\textbf{\color{green} Q2:}}}
The rationale for the style feature space. 
\noindent{\underline{\textbf{\color{green} A2:}}}
As stated in L. 318-321, “Inspired by [38]...”, which uses feature statistics to estimate style space of images, we propose a parallel style feature space for text modality. Its validity is supported by the alignment between text and image feature spaces in the CLIP model. We appreciate your feedback and will clarify this explanation in the revised version.
%s Line 318 “Inspired by []”, as well as other paper about style feature space of images, 再基于clip中的文本模态和图像模态共享特征空间的理论基础，我们仿照图像特征空间合理地提出了文本模态的style feature space并且我们认为它的合理性可以由clip的文本和图像特征空间的一致性来保证。感谢您宝贵的意见，我们将会在文章中增加这个说明来make the风格空间的定义more clear and合理。
\noindent{\underline{\textbf{\color{green} Q3:}}}
Additional comparative experiments. 
\noindent{\underline{\textbf{\color{green} A3:}}}
Thanks! The comparative results are shown in the table below and show that HAM-PEDES also outperforms other datasets based on the RDE method, especially with a 3.45\% Rank-1 improvement over SOTA on RSTP, further demonstrating the effectiveness of our method.
\begin{table}[h]
\vspace{-1em}
\resizebox{0.475\textwidth}{!}{%
\begin{tabular}{c|c|c|c}
\hline
Method & CUHK-PEDES & ICFG-PEDES & RSTPReid \\ \hline
LuPerson-T+RDE & 76.01/67.92  &67.07/40.08  &65.85/51.14  \\ 
SYNTH-PEDES(1.0M)+RDE & 76.23/67.99  &68.19/41.04  &66.35/51.12  \\ 
LUPerson-MLLM(1.0M)+RDE & 77.08/69.17  &68.92/41.67  &69.05/53.67  \\ 
% IRRA+4cap & 73.97  &66.76  &  &  &  &  \\
HAM-PDEDE(1.0M)+RDE &77.99/69.72  & 69.95/42.72  &72.50/55.47  \\ \hline
\end{tabular}}
\vspace{-1.5em}
\end{table}

\noindent{\underline{\textbf{\color{green} Q4:}}}
The parameter settings. 
\noindent{\underline{\textbf{\color{green} A4:}}}
Please refer to our reply to R2Q1 and sincerely hope the experimental results can address your concerns.
\noindent{\underline{\textbf{\color{green} Q5:}}}
The superiority of our method over templates.
\noindent{\underline{\textbf{\color{green} A5:}}}
Thanks for your valuable suggestion! Please refer to our reply to R1Q1 for details. In summary, using templates has key drawbacks: limited quantity, loss of stylistic information(e.g., placeholders like [hairstyle] cannot capture the distinction between [straight shoulder-length black hair] and [black hair]) and reliance on MLLM's inherent bias. In contrast, our method incorporates human-annotated priors and fine-tunes the MLLM to mitigate its biases. We will provide a more detailed explanation in the revised version and hope it clarifies your concerns!
%Additionally, due to the bias in the long-tail data distribution of the MLLM's training corpus, even with different prompts (i.e., templates), the outputs of MLLMs still exhibit wording style bias [DOI:10.48550/arXiv.2409.03025, DOI:10.48550/arXiv.1710.02534]. In contrast, our method leverages human-annotated priors and fine-tunes the MLLM to refine its inherent biases. We will provide a more detailed explanation in the revised version and hope this addresses your concerns!
%感谢您的宝贵建议！在Linexx-xx中我们指出template的缺点是一个是数量有限，另一个是只关注sentence pattern丢失其他风格信息，比如[hairstyle]的填空无法体现[black middle-length hair] 和 [black hair]的区别，且由于llm在训练时长尾数据分布的bias，即使给定不同的prompt（即不同template）mllm的输出依然lead to wording style bias，而我们的方法可以用人类先验基于下游微调来refine inherent bias。我们将在修正版本中给以更详细的解释并希望这能解决你的疑惑！

% Reviewer 3
\noindent{\textbf{\color{orange} Response To R3:}}
\noindent{\underline{\textbf{\color{orange} Q1:}}}
Image modality. 
\noindent{\underline{\textbf{\color{orange} A1:}}}
Thanks for your constructive suggestion! Regarding the image modality, we trained the image encoder of the MLLM in HAM but saw no performance improvement. For example, with LLaVA-1.6, the Rank-1 on CUHK-PEDES was 60.60\% (fixed image encoder) and 59.60\% (trainable image encoder). We attribute this to the fact that training the image encoder will harm generalized knowledge in MLLM. Furthermore, We focused solely on textual style diversity since pedestrian images already capture diverse styles (e.g., angles, clarity, lighting) that aid image encoder generalization, while limited text diversity remains the key factor restricting ReID performance. Hope this clarifies your concerns!
%Thanks for your 有建设性的意见。对于图像模态的挖掘，事实上我们发现在mllm中将image encoder的参数也训练并不能带来性能提升，如实验结果展示（xxx rank1 （fixed)）and xxx，我们认为是放开mlm的image encoder训练会对原本mlm中的泛化知识造成损害。其次我们只对文本风格多样性进行挖掘而没有考虑图像模态是因为，在海量可获得的行人图像中，包含了各种各样的图像风格如不同拍摄视角、清晰度、光照亮度等，which can already help the image encoder to捕获泛化的行人图像特征，相比起来文本注释的风格毕竟单一化才是限制reid模型泛化性能的主要原因。希望这能解决您的疑惑！
\noindent{\underline{\textbf{\color{orange} Q2:}}}
Long text modeling capacity of CLIP. 
\noindent{\underline{\textbf{\color{orange} A2:}}}
The standard CLIP model’s 77-token limit accommodates HAM-PEDES’s 26.1-word average text length. To validate this, we replaced CLIP with Long-clip (134 tokens) on 1M HAM captions and yielded similar Rank-1 accuracy on CUHK (60.60\% vs. 60.72\%), showing no benefit from increasing the text length limit for feature extraction and alignment.
%The standard CLIP model has a default text length limit of 77 tokens, the average text length in HAM-PEDES is 26.1 words, well within this limit. To validate this, we replaced CLIP with Long-clip (up to 134 tokens) to train on our 1M captions and found Rank-1 accuracy on CUHK to be 60.60\% (CLIP) and 60.72\% (Long-clip), indicating that increasing the text length limit does not enhance the extraction and alignment of pedestrian text features.
%标准CLIP默认的文本长度限制是77tokens，而我们统计了HAM-PEDES中的平均文本长度是xx words，which低于clip的文本限制长度，因此用clip的默认文本长度已经足够handle我们的数据集。为了证实这一点我们也用longclip的长文本位置编码方式代替clip在我们的数据集上进行实验，实验结果为cuhk上的rank1为xx（clip） and xx（longclip with text length of 134）表明增加文本长度限制并不会促进行人文本特征的提取和对齐
\noindent{\underline{\textbf{\color{orange} Q3:}}}
Generalization on more  MLLMs. 
\noindent{\underline{\textbf{\color{orange} A3:}}}
To demonstrate our method’s generalization across MLLMs, we applied HAM to MiniCPM-V2.5, in addition to LLaVA-1.6 and Qwen-VL shown in paper. The results, shown in the table below, confirm HAM’s effectiveness on MiniCPM-V2.5, further validating its generalization capability.
\begin{table}[h]
\vspace{-1em}
\resizebox{0.475\textwidth}{!}{%
\begin{tabular}{c|c|c|c}
\hline
Method & CUHK-PEDES & ICFG-PEDES & RSTPReid \\ \hline
static caption & 39.29/35.83  &24.98/9.19  &34.85/25.50  \\
% IRRA+4cap & 73.97  &66.76  &  &  &  &  \\
HAM+KMeans+UPS($K_1=1000,K_2=1000$) &59.14/52.58  & 34.50/17.18  &45.25/33.22  \\ \hline
\end{tabular}}
\vspace{-1.5em}
\end{table}
%To 证明我们的方法对mllm的泛化适用性，除了文中展示的Llava1.6和Qwen-VL的实验性能，我们还在MiniCPM-V2.5上使用了我们的HAM方法，实验结果如下表所示，表格中的‘static tempalte’和‘’含义和表x中的相同。实验结果证明我们的方法在MiniCPM-V2.5上也有适配性，进一步印证了我们方法的泛化性。
\textbf{Finally, we will release all the code and data upon acceptance as promised in the abstract.}
%我们确保我们的代码和数据集将会在文章被接收之后进行公开，以促进社区对t2i reid的进一步深入研究。










% Thanks! We will carefully revise Fig. 2 to make sure all the elements in this figure are both clear and align with our method descriptions.
% %We will add an image-caption module to the diagram in the final version.

% \noindent{\underline{\textbf{\color{cyan} Q2:}}}
% Performance improvement on HOICLIP [76].
% \noindent{\underline{\textbf{\color{cyan} A2:}}}
% Thanks for this constructive comment! 
% In the original submission, we keep all training settings, including the number of training epochs, the same as HOICLIP. Per your request, we have carefully examined the fine-tuning process on HOICLIP. We discover that our DP-HOI pre-training significantly accelerates the convergence of HOICLIP, which means overfitting may occur if we still keep the number of training epochs the same as the original paper. 
% % Therefore, we reduce the number of HOICLIP fine-tuning epochs to 60 and find the performance of ``HOICLIP+Ours'' is promoted to 36.56\%, 34.36\%, and 37.22\% mAP for the full, rare, and non-rare HOI categories, respectively, which are significantly higher than the original HOICLIP model. We will release all code, training logs, and checkpoints of this experiment.
% % As illustrated in Fig. A(a), we reduce the number of HOICLIP fine-tuning epochs to 60 and find the performance of ``HOICLIP+Ours'' is promoted to 36.56\%, 34.36\%, and 37.22\% mAP for the full, rare, and non-rare HOI categories, respectively, which are significantly higher than the original HOICLIP model. 
% As illustrated in Fig. A(a), we reduce the number of HOICLIP fine-tuning epochs to 60 and find the performance of ``HOICLIP+Ours'' is promoted to 36.56\%, 34.36\%, and 37.22\% mAP for the full, rare, and non-rare HOI categories, respectively. 
% % We will release all code, training logs, and checkpoints of this experiment.
% We will release the code and checkpoints of this experiment.
% Moreover, we validate the effectiveness of our method on zero-shot HOI detection in Table 2 of the supplementary. 
% % We improve the performance of HOICLIP by 4.12\% for unseen categories under the RF-UC setting, reaching 29.65\% mAP. 
% We improve the performance of HOICLIP by 4.12\% for unseen categories under the RF-UC setting. 
% The above experimental results indicate that the performance promotion by our method is also significant on HOICLIP.

% % {\small\begin{figure}[h]
% % \vspace{-3.5mm}
% %   \begin{center}
% %   \includegraphics[width=0.95\linewidth]{figures/rebuttal.pdf}
% %   \end{center}
% %   \vspace{-8.2mm}
% %   \label{fig:rebuttal}
% % \end{figure}
% % }
% % {\small\begin{verbatim}
% %    \usepackage{graphicx} ...
% %    \includegraphics[width=0.8\linewidth]
% %                    {myfile.pdf}
% % \end{verbatim}
% \noindent{\underline{\textbf{\color{cyan} Q3:}}}
% Visualizations for DP-HOI.
% \noindent{\underline{\textbf{\color{cyan} A3:}}}
% As illustrated in Fig. A(b), we visualize the attention maps for the last detection decoder layer (the first row) and interaction decoder layer (the second row) of the most confident human query according to RPQ. It can be seen that detection attention maps accurately localize the boundaries of the person and the interaction attention maps accurately localize the regions of interaction. Therefore, with disentangled supervision signals, the two decoders attend to different features for object detection and interaction classification purposes, respectively. 
% % We will add more examples in the final version.
% % We will visualize the attention maps for detection decoder and interaction decoder to illustrate the benefits of DP-HOI intuitively in the final version. The above are some examples. It is shown that with disentangled supervision signals, the two decoders attend to different features for object detection and interaction classification purposes, respectively.


% % Reviewer 2
% \noindent{\textbf{\color{green} Response To R2:}}
% \noindent{\underline{\textbf{\color{green} Q1:}}}
% Performance of HOICLIP on rare categories. 
% \noindent{\underline{\textbf{\color{green} A1:}}}
% Thanks for this constructive comment! Please refer to our reply to Q2 of R1 (Dq8H) for details. In summary, since DP-HOI provides high-quality model weights for initialization, we can reduce fine-tuning epochs from 90 to 60. This reduces overfitting risk and promotes the mAP of HOICLIP on rare HOI categories by as much as 3.24\% mAP, reaching 34.36\% mAP. 
% % We will also release the code of ``HOICLIP+Ours'' to ensure reproducibility.

% \noindent{\underline{\textbf{\color{green} Q2:}}}
% The order of methods in Table 2.
% \noindent{\underline{\textbf{\color{green} A2:}}}
% Thanks! We will modify the order of methods in Table 2 as you suggested.

% \noindent{\underline{\textbf{\color{green} Q3:}}}
% The meaning of HAW.
% \noindent{\underline{\textbf{\color{green} A3:}}}
% HAW refers to using the `A1' database mentioned in L.462 and Table 1. 
% % We will replace `HAW’ with `A1’ in the final version to avoid misunderstanding. 
% We will replace `HAW’ with `A1’ to avoid misunderstanding. 
% % We will also explain that `A1’ denotes using the A1 database in L.470.

% \noindent{\underline{\textbf{\color{green} Q4:}}}
% Weights initialization of QPIC [34].
% \noindent{\underline{\textbf{\color{green} A4:}}}
% % We initialize the first three decoder layers of QPIC according to our pre-trained detection decoder, and the last three decoder layers of QPIC according to our pre-trained interaction decoder. We empirically find this setting achieves the best performance (30.63\% mAP). If we perform model initialization according to our pre-trained detection decoder or interaction decoder only, the mAP drops to 30.24\% and 29.37\%, respectively. We will add these details in the final version.
% We initialize the first three decoder layers according to our pre-trained detection decoder, and the last three decoder layers according to our pre-trained interaction decoder. We empirically find this setting achieves the best performance (30.63\% mAP). If we perform model initialization according to our pre-trained detection decoder or interaction decoder only, the mAP drops to 30.24\% and 29.37\%, respectively.

% \noindent{\underline{\textbf{\color{green} Q5:}}}
% Suggestion on Fig. 2.
% \noindent{\underline{\textbf{\color{green} A5:}}}
% Many thanks for this suggestion! 
% % Thanks!
% We will supplement the arrow from $V_e$ to the interaction decoder in the final version.


% % Reviewer 3
% \noindent{\textbf{\color{orange} Response To R3:}}
% \noindent{\underline{\textbf{\color{orange} Q1:}}}
% Comparisons with RLIPv2 [69].
% \noindent{\underline{\textbf{\color{orange} A1:}}}
% Many thanks for this constructive comment! As the time of rebuttal period is very tight, we scale up the size of pre-training data from 367k to 500k. The new pre-training data are mainly from Kinetics-700.
% With the new pre-trained model weights, the performance on CDN-S\textsuperscript{\dag}+CCS\textsuperscript{$*$} is promoted from 35.38\% to 35.90\% mAP on the full categories of HICO-DET. Moreover, the performance of HOICLIP is promoted from 36.56\% to 36.95\% mAP. In comparison, RLIPv2 employs 1,967k pre-training data and its mAP is 35.38\%. It is clear that DP-HOI outperforms RLIPv2.
% % We will add the above results in the final version of the paper. 

% \noindent{\underline{\textbf{\color{orange} Q2:}}}
% Suggestions on dataset abbreviations.
% \noindent{\underline{\textbf{\color{orange} A2:}}}
% % Thanks! We will replace the nicknames with dataset abbreviations according to your advice.
% Thanks! We will replace the nicknames with dataset abbreviations.

% \noindent{\underline{\textbf{\color{orange} Q3:}}}
% Introduction to positional encoding.
% \noindent{\underline{\textbf{\color{orange} A3:}}}
% Thanks! We follow the DETR paper [9] and utilize fixed sine positional encoding. 
% We will add more details in the final version.

% \noindent{\underline{\textbf{\color{orange} Q4:}}}
% Loss for verb classification.
% \noindent{\underline{\textbf{\color{orange} A4:}}}
% We have cited focal loss [55] and InfoNCE loss [85] for verb prediction in L.327. Their formulas will be added in the final version.

% \noindent{\underline{\textbf{\color{orange} Q5:}}}
% Other implementation details.
% \noindent{\underline{\textbf{\color{orange} A5:}}}
% First, during the training of the Verb Classification Branch, the Transformer Detection Decoder is also trained. We find this strategy does not degrade the detection performance compared with the frozen strategy. Second, for cases where multiple persons perform the same action, RPQ probably makes correct predictions for all humans in the image.
% But we only supervise the query with the most confident predictions according to VPF. In Table 6, we show this strategy outperforms the one supervising all human queries. This is because the latter may introduce noisy supervision for images with complex content. Third, the verb classifier (focal loss,  L.327) is a multi-class classifier. 
% %Please refer to L.336-337 for details. 
% Finally, we will release all the code and checkpoints as promised in the abstract (L.024-025).
% Will the code be made open-source?
% \noindent{\underline{\textbf{\color{cyan} A5:}}}
% As outlined in L.024-025, we will release the code and the pre-trained models.
% \noindent{\underline{\textbf{\color{cyan} Q6:}}}
% Will the Transformer Detection Decoder be trained?
% \noindent{\underline{\textbf{\color{cyan} A6:}}}
% We train without frozen the Transformer Detection Decoder during pre-training, and find it 
% will not compromise  the detection performance.
% \noindent{\underline{\textbf{\color{cyan} Q7:}}}
% Can VPF predict actions of multiple humans?
% \noindent{\underline{\textbf{\color{cyan} A7:}}}
% We supervised the most confident human query by VPF. In Table 6, we show the result of supervised multiple human. This method may introduce noise, which leads to a degradation in performance.
% \noindent{\underline{\textbf{\color{cyan} Q8:}}}
% The details of verb classifier.
% \noindent{\underline{\textbf{\color{cyan} A8:}}}
% We utilized multi-class classifier as our action classifier.






% When placing figures in \LaTeX, it is almost always best to use \verb+\includegraphics+, and to specify the  figure width as a multiple of the line width as in the example below
% {\small\begin{verbatim}
%    \usepackage{graphicx} ...
%    \includegraphics[width=0.8\linewidth]
%                    {myfile.pdf}
% \end{verbatim}
% }


%%%%%%%%% REFERENCES
% {
%     \small
%     \bibliographystyle{ieeenat_fullname}
%     \bibliography{main}
% }

\end{document}

